Unsupervised Training for 3D Morphable Model Regression

We present a method for training a regression network from image pixels to 3D morphable model coordinates using only unlabeled photographs. The training loss is based on features from a facial recognition network, computed on-the-fly by rendering the predicted faces with a differentiable renderer. To make training from features feasible and avoid network fooling effects, we introduce three objectives: a batch distribution loss that encourages the output distribution to match the distribution of the morphable model, a loopback loss that ensures the network can correctly reinterpret its own output, and a multi-view identity loss that compares the features of the predicted 3D face and the input photograph from multiple viewing angles. We train a regression network using these objectives, a set of unlabeled photographs, and the morphable model itself, and demonstrate state-of-the-art results.

==> fig_lfw_inter_cluster.tex <==
\begin{figure}
\centering
\hspace{-0.15cm}{
\includegraphics[width=3.3in]{intra-cluster-bl10.png}} %was 3.1
\label{fig:lfw_inter_cluster}
\caption{Cosine similarity between VGG-Face fc7 layers for all successful matches in LFW. The mean fc7 cosine similarity of all compared methods between input photograph and frontal renderings of output geometry on the MoFA test set is shown superimposed.}
\end{figure}


==> fig_lfw_intra_cluster.tex <==
\begin{figure}
    \centering
    \hspace{-.15cm}{
    \includegraphics[width=3.3in]{inter-cluster-bl10.png}}
    \caption{Cosine similarity between VGG-Face fc7 layers for all pairs of images in LFW of different identities. The mean fc7 cosine similarity of all compared methods between the input photograph and a rendering of output geometry on the MoFA test set is shown superimposed.}
    \label{fig:lfw_intra_cluster}
\end{figure}

==> fig_micc_visualization.tex <==
\begin{figure*}
\includegraphics[width=7in]{micc-box-plot.png}
\caption{MICC Result comparison to Tran et al. on the Cooperative, Indoor, and Outdoor result sets. The 25th-75th percentiles are shaded for each set. Note that our results have lower mean and median errors, are more consistent between subjects, and are more robust to changes in environmental conditions.}
\end{figure*}

==> fig_qualitative_sela_micc.tex <==
% \begin{figure}[t]
% \begin{tabular}{c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c@{\hspace{1mm}}c}

% \vspace{.4em}
% \hspace{-0.7cm}{Input} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/in/1_cropped_input.jpg}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/in/2_cropped_input.jpg}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/in/11_cropped_input.jpg}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/in/12_cropped_input.jpg}}\\
% Sela, et al. (D) &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-depth/1_depth.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-depth/2_depth.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-depth/11_depth.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-depth/12_depth.png}}\\

% Sela, et al. (M) &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-shape/1.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-shape/2.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-shape/11.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/sela-shape/12.png}}\\
% Ours (shape) &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-shape/1.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-shape/2.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-shape/11.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-shape/12.png}}\\
% Ours (color) &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-textured/1.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-textured/2.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-textured/11.png}} &
% \subfloat{\includegraphics[width=0.55in,align=c]{qual-sela/us-textured/12.png}}\\
% \end{tabular}
% \vspace{0.5mm}
% \caption{Comparison to Sela, et al. 2017 on the first male and female faces in the MICC dataset. (D) is the depth image predicted by the network, and (M) is the mesh fit with nonrigid registration.}
% \label{fig:sela-comparison}
% \vspace{-2mm}
% \end{figure}

\begin{figure}[t]
\centering
\begin{tabular}{c@{\hspace{0.8mm}}c@{\hspace{0.8mm}}c@{\hspace{0.8mm}}c@{\hspace{0.8mm}}c}
Input & \multicolumn{2}{c}{Sela et al.\cite{DBLP:journals/corr/SelaRK17}} & \multicolumn{2}{@{\hspace{-0.5mm}}c}{Ours}\\
\toprule
&(D)&(M)&Shape&Color\\
 
\vspace{.2em}
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/in/1_cropped_input.jpg}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-depth/1_depth.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-shape/1.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-shape/1.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-textured/1.png}}\\
\vspace{.2em}

\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/in/2_cropped_input.jpg}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-depth/2_depth.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-shape/2.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-shape/2.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-textured/2.png}}\\
\vspace{.2em}

\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/in/11_cropped_input.jpg}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-depth/11_depth.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-shape/11.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-shape/11.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-textured/11.png}} &
\vspace{.2em}

\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/in/12_cropped_input.jpg}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-depth/12_depth.png}} &
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/sela-shape/12.png}} & 
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-shape/12.png}} & 
\subfloat{\includegraphics[width=0.6in,align=c]{qual-sela/us-textured/12.png}}\\

\end{tabular}
\vspace{0.1mm}
\caption{Comparison to Sela et al. \cite{DBLP:journals/corr/SelaRK17} on the first male and female faces in the MICC dataset. (D) is the depth image predicted by the network, and (M) is the mesh fit with nonrigid registration.}
\label{fig:sela-comparison}
%\vspace{-2mm}
\end{figure}

==> table_bias_and_variance.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{lcccc}
%     \toprule
%     Method & Shape Bias & Shape Stddev. & Color Bias & Color Stddev\\
%     \midrule
%     \tran & 0.46 & 0.36 & 0.67 & \textbf{0.54}\\
%     \ours & \textbf{0.24} & \textbf{0.41} & \textbf{0.42} & 0.50\\ % Revision: Batch-reg v1, first 99 parameters.
%     \bottomrule
%     \end{tabular}
%     \caption{Model Variance \& Bias on LFW.}
%     \label{tab:varandbias}
% \end{table*}

\begin{table}
\centering
\begin{tabular}{lcc|cc}
\toprule
& \multicolumn{2}{c|}{Shape} & \multicolumn{2}{c}{Color}\\
Method & Bias & Std. Dev. & Bias & Std. Dev.\\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\tran & 0.46 & 0.36 & 0.67 & 0.54\\
\ours & \textbf{0.45} & \textbf{0.56} & \textbf{0.57} & \textbf{0.73}\\ % Revision: bl10, first 99 parameters
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{Model Variance \& Bias on LFW.}
\label{table:varandbias}
\end{table}

==> table_vgg_face_cosine_similarity.tex <==
\begin{table}
\centering
% Results versions: batch-reg v1
\begin{tabular}{lccc}
\toprule
Method & LFW & MICC-Coop & MoFA-Test \\
\midrule
% Our micc revision: nov8
% Our mofa revision: bl10
% Others: batch-reg
\mofa & $-$ & $-$ & 0.181\\
\tran & 0.161 & 0.163 & 0.215\\
\ours & \textbf{0.347} & \textbf{0.411} & \textbf{0.403}\\
\bottomrule
\end{tabular}
\vspace{0.5em}
\caption{Cosine similarity between VGG Face $\phi(\ell_t)$ layers for input images and front-view renderings of network outputs.}
%\vspace{-1.2em}
\label{table:vggface}
\end{table}
